Generalization and Stability of Interpolating Neural Networks with Minimal Width

We investigate the generalization and optimization properties of shallow neural-network classifiers trained by gradient descent in the interpolating regime. Specifically, in a realizable scenario where model weights can achieve arbitrarily small training error $\epsilon$ and their distance from initialization is $g(\epsilon)$, we demonstrate that gradient descent with $n$ training data achieves training error $O(g(1/T)^2 /T)$ and generalization error $O(g(1/T)^2 /n)$ at iteration $T$, provided there are at least $m=\Omega(g(1/T)^4)$ hidden neurons. We then show that our realizable setting encompasses a special case where data are separable by the model's neural tangent kernel. For this and logistic-loss minimization, we prove the training loss decays at a rate of $\tilde O(1/ T)$ given polylogarithmic number of neurons $m=\Omega(\log^4 (T))$. Moreover, with $m=\Omega(\log^{4} (n))$ neurons and $T\approx n$ iterations, we bound the test loss by $\tilde{O}(1/n)$. Our results differ from existing generalization outcomes using the algorithmic-stability framework, which necessitate polynomial width and yield suboptimal generalization rates. Central to our analysis is the use of a new self-bounded weak-convexity property, which leads to a generalized local quasi-convexity property for sufficiently parameterized neural-network classifiers. Eventually, despite the objective's non-convexity, this leads to convergence and generalization-gap bounds that resemble those found in the convex setting of linear logistic regression.

==> notes.tex <==
\section{Notes}


\subsection{Comments}

\paragraph{Assumption \ref{ass:loss second order self boundedness}} This assumption is not needed other than for exponential loss for which you use it to show descend lemma. Since it is not critical for any of the main results I would not state. Instead, it makes more sense to me to assume smoothness and add a remark that for the exponential loss smoothness is essentially substituted by second-order self-boundedness.

\paragraph{Definition \ref{defn:sbhs}.} Alternative name: Self-bounded weak convexity. I think it is more specific and descriptive than ``Hessian spectrum.'' Also suggestive of how the property is used in the proofs

\paragraph{Title.} I recommend ``... neural-network classifiers'' instead of ``.. neural-networks.'' I understand dropping the word ``shallow'' but ``classification'' is in my opinion a fair description of the work otherwise I find the title unecessarily generic

\paragraph{Definition \ref{defn:self-bounded}.} There is no use of this in the paper. I recommend removing or at least only keeping the first order (following comment above)

\paragraph{Realizability.} It looks to me that all results can be stated in terms of realizability assumption (or what you call NN-Realizability). Theorems can and should be stated in terms of $\epsilon$ and $\rho(\epsilon):=f^{-1}(\epsilon)/\delta$. The result is then more general. Besides, right now it is not clear what loss function Theorem \ref{thm:gengap} holds for. Another advantage of this is that we can also have a corollary for polynomial loss. see below

\paragraph{Other losses.} It looks to me that you can handle any loss that is self-bounded. This includes the polynomially-tailed loss, sub and super exponential tailed losses in \cite{pmlr-v178-schliserman22a}. So worth stating a general result in terms of realizability + self-boundedness. (I thought a bit wether possible to extend to $\delta$-self bounded as in \cite{pmlr-v178-schliserman22a} but is more tricky here).

\paragraph{Homogeneity.} What is the role of the homogeneity constant $k$? Perhaps we should think that it might be unnecessarily complicating the statements without really adding any new insights? Of course it doesn't hurt but it can be a bit confusing if some remarks, even theorems (e.g. main Theorem 3) are stated assuming $k=1$ without explicit mention.

\subsection{Technical comparisons to most-closely related works}

\paragraph{Self-boundedness.}
The self-boundedness assumption (Assumption \ref{ass:loss self boundedness}) is key to our proof. This remark details its origin and distinguishes its use in our paper from prior works. The use of this property for logistic/exponential loss to bound training/generalization error has been seen in previous works \cite{}. \citet{pmlr-v178-schliserman22a} were the first to apply it for stability analysis of linear classifiers, using it to improve a bound by \citet{lei2020fine} on the leave-one-out model-stability term in terms of the training error. They also generalized the self-boundedness assumption to $\abs{f^\prime(t)}\leq (f(t))^{1-\zeta}$ for $\zeta\in[0,1/2]$, with Assumption \ref{ass:loss self boundedness} as a special case ($\zeta=0$), and used it to find new bounds on test loss for various losses including polynomial-decaying and sub/super-exponential. Our work is the first to use self-boundedness for stability analysis of more complex nonlinear shallow neural-network classifiers. Unlike the simpler linear case of \citet{pmlr-v178-schliserman22a}, its use in our paper is more critical in various parts of the proof, particularly for (i) our non-expansiveness bound on GD and (ii) our training error bound, both of which use the newly defined self-bounded weak convexity property (see Definition \ref{defn:sbhs}). In contrast, in \cite{pmlr-v178-schliserman22a}, (i) and (ii) follow easily due to the empirical loss function being convex.


% The assumption of self-boundedness (Assumption \ref{ass:loss self boundedness}) is crucial to our proof. This remark explores its origin and how its use in our paper differs from prior works. The use of this property, specifically applied for logistic/exponential loss, has been used in several previous works for bounding training/generalization error under various settings  \cite{}. To the best of our knowledge, \citet{pmlr-v178-schliserman22a} were the first to utilize this property for stability analysis of linear classifiers. Specifically, they used it to improve an earlier bound by \cite{lei2020fine} on the on-average leave-one-out (LOO) model-stability term as a function of the training error. \citet{pmlr-v178-schliserman22a} also formalized a more general version of self-boundedness assumption $\abs{f^\prime(t)}\leq (f(t))^{1-\zeta}$ for $\zeta\in[0,1/2]$, with Assumption \ref{ass:loss self boundedness} being a special case ($\zeta=0$), and used it to obtain new bounds on test loss for various losses including polynomial-decaying and sub/super-exponential. Our work utilizes for the first time the self-boundedness assumption for stability analysis of (nonlinear) shallow neural-network classifiers. Unlike the linear case of \cite{pmlr-v178-schliserman22a}, its use in our paper is more crucial entering various parts of the proof. Concretely, it is crucial for (i) our bound on the non-expansiveness of GD and (ii) our bound on the training error. In both cases, the assumption comes into the game via invoking the newly defined self-bounded weak convexity property.  In contrast both (i) and (ii) follow easily in the setting of \cite{pmlr-v178-schliserman22a} by convexity of the empirical loss function.

\paragraph{Stability-analysis framework for shallow neural nets.} In terms of techniques, The most closely related works to our paper  are the recent works \cite{richards2021learning,richards2021stability,leistability}, which also utilize the stability-analysis framework to derive test-loss bounds of GD for shallow neural networks. 

\citet{richards2021learning} investigates the generalization gap of weakly-convex losses for which $\lambda_{\min}(\nabla^2 \hat{F}(w))\geq - \epsilon$ for a constant $\epsilon>0.$ Note by Lemma \ref{lem:gradients_and_hessians_bounds_general} that our empirical loss is weakly convex with $\epsilon=LR^2G_f/\sqrt{m}$ since the logistic loss is $G_f$-Lipschitz. Within the stability analysis framework, \citet{richards2021learning} leverage the weak-convexity property to establish an approximate expansiveness property of GD iterates that in our setting translates to
\begin{align}
    \left\|\left(w-\eta\nabla\hat{F}(w)\right)-\left(\wpr-\eta\nabla\hat{F}(\wpr)\right)\right\|\lesssim\left(1+\frac{\eta LR^2 G_f}{\sqrt{m}}\right)\left\|w-\wpr\right\|\,.
    \label{eq:RichardsRabbat}
\end{align}
When using this inequality to bound the model stability term at iteration $t$, and in order to obtain non-vacuous bounds, the extra term in \eqref{eq:RichardsRabbat} must be chosen such that ${\eta LR^2 G_f}{\sqrt{m}}\lesssim 1/t$. This leads to polynomial-width parameterization requirement $m\gtrsim t^2$. In this work, we reduce the requirement to logarithmic  $m\gtrsim \log(t)$, by significantly tightening \eqref{eq:RichardsRabbat}. This is achieved by introducing two crucial ideas. The first is to exploit the self-boundedness property of the logistic loss, which yields a stronger \emph{self-bounded} weak convexity $\lambda_{\min}(\nabla^2 \hat{F}(w))\geq - LR^2\hat{F}(w)/\sqrt{m}.$ With this, we show in Corollary \ref{cor:9.1} that
\begin{align}
\left\|\left(w-\eta\nabla\hat{F}(w)\right)-\left(\wpr-\eta\nabla\hat{F}(\wpr)\right)\right\|\leq\left(1+\frac{\eta LR^2}{\sqrt{m}}\max_{\alpha\in[0,1]}\hat{F}(\wa)\right)\left\|w-\wpr\right\|\,\label{eq:Hossein}
\end{align}
for some $\wa=\alpha w+(1-\alpha)\wpr$. Our second idea comes into bounding the term $\max_{\alpha\in[0,1]}F(\wa)$ which in our bound replaces the Lipschitz constant $G_f$  of \eqref{eq:RichardsRabbat}. To control $\max_{\alpha\in[0,1]}F(\wa)$, we identify and use the Generalized Local Quasi-convexity of Proposition \ref{propo:GLQC}. This replaces $\max_{\alpha\in[0,1]}F(\wa)$ in \eqref{eq:Hossein} with $\tau\cdot \max\{\hat F(w),\hat F(\wpr)\}$ for $\tau\approx 1+LR^2\|w-w'\|^2/\sqrt{m}$ and note that we can guarantee $\tau=O(1)$  provided $\sqrt{m}\gtrsim \max\{\|w\|^2,\|\wpr\|^2\}.$ Now, in order to bound the model stability term, we apply non-expansiveness for GD iterate $w=w_t$ and its leave-one-out counterpart $w=w_t^\negi$: Provided $m\gtrsim \max\{\|w_t\|^4,\|w_t^\negi\|^4\}\approx (\log(t))^8,$
\begin{align}
\left\|\left(w_t-\eta\nabla\hat{F}(w_t)\right)-\left(w_t^\negi-\eta\nabla\hat{F}(w_t^\negi)\right)\right\|&\lesssim\left(1+\frac{\eta LR^2}{\sqrt{m}} \max\{\hat F(w),\hat F(\wpr)\} \right)\left\|w-\wpr\right\|\,\nn
\\
&\lesssim\left(1+\frac{\eta LR^2}{t\,\sqrt{m}}  \right)\left\|w-\wpr\right\|\
\label{eq:Hossein2}
\end{align}
Compared to \eqref{eq:RichardsRabbat} note in \eqref{eq:Hossein2} that the extra term is already of order $1/t$. Hence, the only parameterization requirement is $m\gtrsim \max\{\|w_t\|^4,\|w_t^\negi\|^4\}\approx (\log(t))^8.$ 
While the above describes our main technical novelty compared to \cite{richards2021learning}, our results surpass theirs in other aspects. Specifically, we also obtain tighter bounds on the optimization error, again thanks to leveraging self-bounded properties of the logistic loss. Overall, for the separable setting, we show a $\tilde{O}(1/n)$ test-loss bound compared to $O(1/\sqrt{n})$ in their paper. 

In closing, we remark that our logarithmic width requirements and expansiveness bounds are also significantly tighter than those that appear in \cite{richards2021stability,leistability}. While their results are not directly comparable to ours as they only apply to square-loss functions, we reference them here for completeness: \citet{richards2021stability} upper-bounds the expansiveness term on the left-hand side of \eqref{eq:Hossein2} by $\lesssim \left(1+\eta\sqrt{\eta t}/\sqrt{m}\right)$ which requires $m\gtrsim t^3$ so that is of order $1+1/t$. More recently, \citet{leistability} slightly modifies their bound to $\lesssim \left(1+\eta({\eta t})^{3/2}/(n\sqrt{m})\right)$ which requires $m\gtrsim (\eta t)^5/n^2.$



% $\frac{1}{n}\sum x_i$
